Single Past Null Geodesic in the Lemaitre-Tolman-Bondi Cosmology

This work provides a general discussion of the spatially inhomogeneous Lema\^itre-Tolman-Bondi (LTB) cosmology, as well as its basic properties and many useful relevant quantities, such as the cosmological distances. We apply the concept of the single null geodesic to produce some simple analytical solutions for observational quantities such as the redshift. As an application of the single null geodesic technique, we carry out a fractal approach to the parabolic LTB model, comparing it to the spatially homogeneous Einstein-de Sitter cosmology. The results obtained indicate that the standard model, in this case represented by the Einstein-de Sitter cosmology, can be equivalently described by a fractal distribution of matter, as we found that different single fractal dimensions describe different scale ranges of the parabolic LTB matter distribution. It is shown that at large ranges the parabolic LTB model with fractal dimension equal to 0.5 approximates the matter distribution of the Einstein-de Sitter universe.

==> app1/app1.tex <==
% ********** Appendix 1 **********
\chapter{Appendix}
\label{sec:appendix1}

... some text ...

% ********** End of appendix **********


==> chap3 <==
% ********** Chapter 2 **********
\chapter{The Lema\^itre-Tolman-Bondi Geometry}
\label{chapter1}

\section{The Field Equation Solutions}

The Einstein Field Equations of General Relativity, given by

\begin{equation}
	G^{\mu \nu} = R^{\mu \nu} - \frac{1}{2}g^{\mu \nu}R = \frac{8 \pi G}{c^4}T_{\mu \nu} \label{einstein equations}
\end{equation}

are the equations that define the relationship between the geometry and the distribution of matter in the Universe. They are the results of Einstein's search for the ultimate gravitational theory to describe the matter dynamics in space-time.

The right-hand side of the equation (\ref{einstein equations}) is the "geometry side", represented by the Einstein tensor. The Einstein tensor is composed of a combination of contractions of the Riemann tensor, as can be seen in equation (\ref{einstein equations}). The Riemann tensor is a combination of second (covariant) derivatives of the metric tensor. This side of the equation shows how the content of the left-hand side of the equation is going to move in the chosen space-time coordinates.

The left-hand side of the equation (\ref{einstein equations}) is the "matter side", because the quatity $ T_{\mu \nu} $ is the matter-radiation tensor. It defines what will be interacting and moving in the space-time defined in the right-hand side of the equation.

The resulting equations, when the metric and matter-radiation tensor are defined, are going to show how the space-time is altered by the mass-radiation content, and vice-versa. Under certain assumptions, the equations can be solved so that the result is a description of the space-time and matter-radiation content.

For the LTB model, some of these assumptions are the following

-The coordinates of the space-time are defined as comoving coordinates; \\


-The coordinates of the space-time are defined as synchronous coordinates; \\


-The space-time is spherically simetric; \\


-The fluid given by the matter-radiation tensor is perfect (rotation zero). \\


Then the Einstein tensors are given by \\



%\begin{equation}

%\end{equation}

with the assumed equation of state $ p = 0 $, i.e. evolution by gravitation only. This happens because if it is assumed that the equation of state is given by some function $ f(p) $, then the entropy per particle is going to be a universal constant (...). With $ R' \neq 0 $ the result is
\\
----------------- \\
%\begin{equation}

and the final main field equation is

\begin{equation}
	R'^2 = 2E(r) + 2\frac{M(r)}{R} \label{fieldeq1}
\end{equation}

This equation has the same form as the energy equation for a Newtonian radial motion in a Coulomb potential. The terms in the equation can be interpreted while doing this analogy, with the term $ c^2M(r)/G $ being as a active gravitational mass, and the term $ c^2E(r)/G $ playing the role of the total energy within the shell of radius $ r $.

The second field equation will give the definition of the mass density in this geometry,

\begin{equation}
	\frac{8 \pi G}{c^4} = \frac{2M'}{R^2R'} \label{fieldeq2}
\end{equation}

It can be seen that there are two singularities arising from these equations. One of them occurs when $ R = 0 \neq M'(r) $, and is interpreted as the Big Bang singularity. The other one comes where $ R' = 0 \neq M'(r) $, and it defines a shell crossing singularity, where the mass density goes to infinity and becomes negative. These two singularities can be avoided by an appropiate choice of the functions of the model, M(r), E(r), and a third arbitrary function, $ t_B(r) $. This last function appears as a constant of integration when the equation (\ref{fieldeq1}) is integrated. It defines the big bang time, which in this geometry is position-dependent.

The final solution for the metric is then

\begin{equation}
		ds^2 = dt^2 - \frac{R'^2}{1+ 2E(r)}dr^2 - R^2(t,r)(d\theta^2 + sin^2\theta d\phi^2) \label{metricLTori}
\end{equation}

where R(r,t) is determined by the equation (\ref{fieldeq1}). This metric defines what is called the Lema\^itre-Tolman-Bondi model. This solution was first found by Lema\^itre in 1933, then reinterpreted by Tolman in 1934 and by Bondi in 1947. 

%Some reference~\cite{Led2004}

%Some symbols: DMC\label{sym:DMC}, LZ77\label{sym:LZ77}, LZ78\label{sym:LZ78}.

% ********** End of chapter **********


==> chap4 <==
% ********** Chapter 2 **********
\chapter{The Unique Null Geodesic}
\label{chapter2}

\section{The Concept}



%Some reference~\cite{Led2004}

%Some symbols: DMC\label{sym:DMC}, LZ77\label{sym:LZ77}, LZ78\label{sym:LZ78}.

% ********** End of chapter **********


==> symbols.tex <==
% *************** List of symbols and abbreviations ***************

% ******************************************************************************
% You can make list of symbols and abbreviations here.
% You only need to make a label when a symbol is introduced in the document and
% here you can reference this label to obtain page number.
% ******************************************************************************

\chapter[List of Symbols and Abbreviations]{List of Symbols\\ and Abbreviations}

\begin{center}
\small
\begin{longtable}{lp{3.0in}c}
\toprule
\multicolumn{1}{c}{Abbreviation}
                & \multicolumn{1}{c}{Description}
                                & \multicolumn{1}{c}{Definition}\\ \midrule\addlinespace[2pt] \endhead
\bottomrule\endfoot
DMC				& dynamic Markov coder
                                & \pref{sym:DMC}\\
LZ77			& kind of Ziv--Lempl algorithms
                                & \pref{sym:LZ77}\\
LZ78			& kind of Ziv--Lempel algorithms
                                & \pref{sym:LZ78}\\
\end{longtable}
\end{center}

% *************** End of list of symbols and abbreviations ***************

